DAFA: Distance-Aware Fair Adversarial Training

The disparity in accuracy between classes in standard training is amplified during adversarial training, a phenomenon termed the robust fairness problem. Existing methodologies aimed to enhance robust fairness by sacrificing the model's performance on easier classes in order to improve its performance on harder ones. However, we observe that under adversarial attacks, the majority of the model's predictions for samples from the worst class are biased towards classes similar to the worst class, rather than towards the easy classes. Through theoretical and empirical analysis, we demonstrate that robust fairness deteriorates as the distance between classes decreases. Motivated by these insights, we introduce the Distance-Aware Fair Adversarial training (DAFA) methodology, which addresses robust fairness by taking into account the similarities between classes. Specifically, our method assigns distinct loss weights and adversarial margins to each class and adjusts them to encourage a trade-off in robustness among similar classes. Experimental results across various datasets demonstrate that our method not only maintains average robust accuracy but also significantly improves the worst robust accuracy, indicating a marked improvement in robust fairness compared to existing methods.

==> backup.tex <==

% CCR 수식

\begin{equation}
\label{eq:method_trades_loss_ccr}
{\mathcal{L}}(\beta;\bm{x},y)=\frac{\mathcal{L}_{nat}(\bm{x},y)+\beta_{y}\underset{\norm{\bm{x} - \bm{x}'} \leq \epsilon}{\max}\mathcal{L}_{bndy}(f(\bm{x}), f(\bm{x}'))}{1+\beta_{y}}, 
\smalltab \text{where} \smalltab 
\beta_{y} \leftarrow (\lambda_{CCR} + t_{y}) \cdot \beta.
\end{equation}

%% 이전 세팅 증명


\begin{proof}
binary classification task에서 두 distribution의 classify하는 optimal $\bm{w}$를 구하는 것은 다음과 같이 각 distribution의 평균을 $\frac{1-\alpha}{2}$만큼 평행이동시킨 distribution에 대한 optimal $\bm{w}$와 $b$를 구하는 것과 동일하다. 따라서,
\begin{equation} \label{}
\begin{gathered}
    \mathnormal{y}\stackrel{u.a.r}{\sim} \{-1, +1\}, \smalltab 
    \theta=(\eta, 2\eta, \cdots, d\eta),    
    \tab 
    \bm{\mathnormal{x}} {\sim}
    \begin{cases}
    \mathcal{N}(\frac{1+\alpha}{2}\theta, 1), & \text{if } \mathnormal{y}=+1 \\
    \mathcal{N}(-\frac{1+\alpha}{2}\theta, 1), & \text{if } \mathnormal{y}=-1 \\
    \end{cases}
\end{gathered}
\end{equation}
여기서, $\mathcal{R}_{nat}(f_{nat}|y=+1) + \mathcal{R}_{nat}(f_{nat}|y=-1)$을 최소화하는 값은 $\bm{w}_{nat}=\frac{1}{\lambda_{nat}}\theta$ 그리고 $b=0$이다. 그리고, $0<\epsilon<d\eta$에 대해, $\mathcal{R}_{rob}(f_{rob}|y=+1) + \mathcal{R}_{rob}(f_{rob}|y=-1)$을 최소화하는 값은 $\bm{w}_{rob}=\frac{1}{\lambda_{rob}}\text{max}(\frac{1+\alpha}{2}\theta-\epsilon, 0)$ 그리고 $b=0$이다. $\lambda_{nat},\lambda_{rob}$은 $\norm{\bm{w}}=1$를 만족시키는 값. 이 때 the difference between $\mathcal{R}_{nat}(f_{rob}|+1)$ and $\mathcal{R}_{nat}(f_{nat}|+1)$ is

\begin{align}
\mathcal{R}_{nat}(f_{rob}|+1) - \mathcal{R}_{nat}(f_{nat}|+1) &= Pr.(\bm{w}_{rob}^\top \bm{\mathnormal{x}} < 0|y=+1)-Pr.(\bm{w}_{nat}^\top \bm{\mathnormal{x}} < 0|y=+1)
\end{align}

\begin{align}
&= Pr.\bigg(\mathcal{N}(0,1)<\frac{\eta\big(\frac{d(d+1)}{2}-\frac{m(m+1)}{2})\big)}{\sqrt{\frac{d(d+1)(2d+1)}{6}-\frac{m(m+1)(2m+1)}{6}}}\bigg) - Pr.\bigg(\mathcal{N}(0,1)<\frac{\eta\big(\frac{d(d+1)}{2})\big)}{\sqrt{\frac{d(d+1)(2d+1)}{6}}}\bigg).
\end{align}
\label{eq:prob_difference_distance}
여기서, $m$은 $m + 1 > \epsilon$을 만족하는 minimum $m$. $m$ is monotone decreasing at $\alpha$. Let $g=\frac{\eta\big(\frac{d(d+1)}{2}-\frac{m(m+1)}{2})\big)}{\sqrt{\frac{d(d+1)(2d+1)}{6}-\frac{m(m+1)(2m+1)}{6}}}$ is monotone decreasing at $m$ because the derivative of this function for $m$ is $\frac{d}{dm}g = -\frac{\sqrt{\frac{3}{2}} \left( d^2 (8 m + 4) + d (2 m^2 + 10 m + 5) + 2 m^3 + 4 m^2 + 3 m + 1 \right)}{2 (2 d^2 + d (2 m + 3) + 2 m^2 + 3 m + 1) \sqrt{2 d^3 + 3 d^2 + d - m (2 m^2 + 3 m + 1)}} <0$ for $0<m<d$. 즉, 미분 연쇄법칙에 의해 $g$ is monotone increasing at $\alpha$. Let 확률 밀도 함수 $\Phi(\mathnormal{x})=Pr.(\mathcal{N}(0,1)<\mathnormal{x})$. Then, function $h(x)=\Phi(\mathnormal{y})-\Phi(\mathnormal{x})$ is monotone decreasing at $x$, where $x < y$. $\mathcal{R}_{nat}(f_{rob}|+1) - \mathcal{R}_{nat}(f_{nat}|+1)=h(g(\alpha))$이므로 미분 연쇄법칙에 의해 the difference between $\mathcal{R}_{nat}(f_{rob}|+1)$ and $\mathcal{R}_{nat}(f_{nat}|+1)$ is monotone decreasing at $\alpha$.


%%%% R(-1) backup

In turn, the derivative with respect to $\alpha$ for the equation \ref{eq:appendix_std_error_neg} is:
\begin{align}
\frac{\partial}{\partial \alpha}\mathcal{R}_{nat}(f_{nat}|-1) &= \text{exp}(z_{-1})\bigg( \frac{1}{\sigma} \cdot \frac{A}{2}\eta - \frac{\frac{A^2}{2}\eta\big(\frac{1+\alpha}{2}\eta\big)}{\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}}} \bigg) \\
&= \text{exp}(z_{-1})\bigg(\frac{\frac{A}{2}\eta\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}} - \sigma\frac{A^2}{2}\eta\big(\frac{1+\alpha}{2}\eta\big)}{\sigma\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}}} \bigg) \\
&= \text{exp}(z_{-1})\bigg(\frac{\frac{A}{2}\eta\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}} - \sigma\frac{A}{2}\eta \sqrt{A^2\big(\frac{1+\alpha}{2}\eta\big)^2}}{\sigma\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}}} \bigg) \\
& \leq \text{exp}(z_{-1})\bigg(\frac{\frac{A}{2}\eta\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2} - \sigma\frac{A}{2}\eta \sqrt{A^2\big(\frac{1+\alpha}{2}\eta\big)^2}}{\sigma\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}}} \bigg) \\
&= \text{exp}(z_{-1})\bigg(\frac{\frac{A}{2}\eta\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2} - \sigma\frac{A}{2}\eta \sqrt{A^2\big(\frac{1+\alpha}{2}\eta\big)^2}}{\sigma\sqrt{A^2 \big(\frac{1+\alpha}{2}\eta\big)^2+\frac{2\sigma^2\log\sigma}{\sigma^2-1}}} \bigg) \\
\end{align}


%%%%%





==> fig/fig_intro_confusion_matrix.tex <==
\begin{wrapfigure}[13]{R}{0.3\linewidth} % control 22
\begin{center}
% \vskip -12mm
% \setlength{\belowcaptionskip}{-1.8\baselineskip}
\raisebox{0pt}[\dimexpr\height-1.5\baselineskip\relax]{\includegraphics[width=1.0\linewidth]{_fig/_fig_method_aaa_matrix.pdf}}% -0.6
% \includegraphics[width=1.0\linewidth]{Figure/biamat_ratio.pdf}
\end{center}
\vskip -2mm
\caption{The confusion matrix of the robust classifier for CIFAR-10.}
\label{fig:method_aaa_matrix}
\end{wrapfigure}

==> fig/fig_method_accuracy_correlation.tex <==
\begin{wrapfigure}[10]{R}{0.3\linewidth} % control 22
\begin{center}
% \vskip -12mm
% \setlength{\belowcaptionskip}{-1.8\baselineskip}
\raisebox{0pt}[\dimexpr\height-1.5\baselineskip\relax]{\includegraphics[width=1.0\linewidth]{_fig/_fig_method_accuracy_correlation.pdf}}% -0.6
% \includegraphics[width=1.0\linewidth]{Figure/biamat_ratio.pdf}
\end{center}
% \vskip -2mm
\caption{The schematic illustration of easy ($x_2$) and hard examples ($x_1$).}
\label{fig:method_accuracy_correlation}
\end{wrapfigure}

==> fig/fig_method_diff_aaa_std_matrix.tex <==
\begin{wrapfigure}[10]{R}{0.3\linewidth} % control 22
\begin{center}
% \vskip -12mm
% \setlength{\belowcaptionskip}{-1.8\baselineskip}
\raisebox{0pt}[\dimexpr\height-1.5\baselineskip\relax]{\includegraphics[width=1.0\linewidth]{_fig/_fig_method_diff_aaa_std_matrix.pdf}}% -0.6
% \includegraphics[width=1.0\linewidth]{Figure/biamat_ratio.pdf}
\end{center}
% \vskip -2mm
\caption{The schematic illustration of easy ($x_2$) and hard examples ($x_1$).}
\label{fig:method_diff_aaa_std_matrix}
\end{wrapfigure}

==> fig/fig_method_diff_eps_accuracy.tex <==
\begin{figure}[t]
% \subfloat[\label{fig:introduction_tsne_clsall}]{
% \includegraphics[width=0.32\linewidth]{_fig/_fig_introduction_tsne_cls_from_trades110.pdf}}
%\hfill
\subfloat[\label{fig:method_eps0_8_accuracy}]{
\includegraphics[width=0.32\linewidth]{_fig/_fig_method_eps0_8_accuracy.pdf}
}
\hfill
\subfloat[\label{fig:method_eps8_0_accuracy}]{
\includegraphics[width=0.32\linewidth]{_fig/_fig_method_eps8_0_accuracy.pdf}}
\hfill
\subfloat[\label{fig:method_eps6_6_bird_cat_accuracy}]{
\includegraphics[width=0.32\linewidth]{_fig/_fig_method_eps6_6_bird_cat_accuracy.pdf}}


\caption{(a) and (b) display the clean and robust accuracy results of the TRADES model, in which half of the classes have a training adversarial budget of 
 $\epsilon=0$, while the remaining classes have a training adversarial budget of $\epsilon=8$. In (a),he first half of the CIFAR-10 dataset classes (0,1,2,3,4) have $\epsilon=0$, while in (b), the latter half of the classes (5,6,7,8,9) have $\epsilon=0$. (c) illustrates the results of three models trained on a binary classification task between the bird and cat classes from CIFAR-10 using the TRADES methodology. Each model was assigned varying training adversarial budgets per class, while the test adversarial budget was consistently set at $\epsilon=6$.}

% \vskip -2mm
%\end{center}
\label{fig:method_diff_eps_accuracy}
\end{figure}


==> fig/fig_method_distribution_var_dist.tex <==

\begin{wrapfigure}[10]{R}{0.3\linewidth} % control 22
\begin{center}
\vskip -4mm
% \setlength{\belowcaptionskip}{-1.8\baselineskip}
\raisebox{0pt}[\dimexpr\height-1.5\baselineskip\relax]{\includegraphics[width=1.0\linewidth]{_fig/_fig_method_gaussian_distribution_v2.pdf}}% -0.6
% \includegraphics[width=1.0\linewidth]{Figure/biamat_ratio.pdf}
\end{center}
% \vskip -2mm
\caption{The schematic illustration of the variance and distance.}
\label{fig:method_distribution_var_dist}
\end{wrapfigure}

==> fig/fig_method_various_confustion_matrix.tex <==
\begin{wrapfigure}[13]{R}{0.3\linewidth} % control 22
\begin{center}
% \vskip -12mm
% \setlength{\belowcaptionskip}{-1.8\baselineskip}
\raisebox{0pt}[\dimexpr\height-1.5\baselineskip\relax]{\includegraphics[width=1.0\linewidth]{_fig/_fig_method_dist_matrix.pdf}}% -0.6
% \includegraphics[width=1.0\linewidth]{Figure/biamat_ratio.pdf}
\end{center}
\vskip -2mm
\caption{Distances between classes of CIFAR-10 in the robust classifier.}
\label{fig:method_dist_matrix}
\end{wrapfigure}

==> table/tab_backup.tex <==
\begin{table}[t]
%\begin{adjustwidth}{-0.25in}{-0.25in}
\caption{Performance of the models for mitigation methods. The best results are indicated in bold. }
\centering
\begin{tabular}{cl|cccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Arch.}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} &
\multicolumn{2}{c|}{Clean} & \multicolumn{2}{c}{Robust} 
\\
& & \multicolumn{1}{c}{Average} & \multicolumn{1}{c|}{Worst} & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Worst} 
\\
\midrule[.05em]
\multirow{4}{*}{ResNet-18}    
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    \midrule[.1em]
\multirow{4}{*}{PRN-18}    
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    \midrule[.1em]
\multirow{4}{*}{WRN-28}    
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
    & TRADES & 0.0 & 0.0 & 0.0 & 0.0 \\
\midrule[.1em]
\end{tabular}
\label{tab:experiment_all110_main_2}
\vskip -5mm
\end{table}


\begin{table}[t]
%\begin{adjustwidth}{-0.25in}{-0.25in}
\caption{Performance of our method in various architectures. The best results among robust fairness methods are indicated in bold. }
\centering
\begin{tabular}{l|ccc|ccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} &
\multicolumn{2}{c}{Clean} & & \multicolumn{2}{c}{Robust}
\\
\multicolumn{1}{c|}{} & (Average) & (Worst) & $\rho_{nat}$ & (Average) & (Worst) &$\rho_{rob}$
\\
\midrule[.05em]
    TRADES & 82.04 $\pm$ 0.10 & 65.70 $\pm$ 1.32 & 0.00 
    & 49.80 $\pm$ 0.18 & 21.31 $\pm$ 1.19 & 0.00 \\
    \midrule[.05em]
    TRADES + FRL & 83.91 $\pm$ 0.33 & \textbf{72.28 $\pm$ 2.33} & \textbf{0.08}
    & 47.00 $\pm$ 0.32 & 27.95 $\pm$ 1.54 & 0.37 \\
    TRADES + BAT & \textbf{86.68 $\pm$ 0.25} & 72.04 $\pm$ 1.88 & 0.04 
    & 45.94 $\pm$ 0.74 & 17.59 $\pm$ 1.83 & -0.19 \\
    TRADES + CFA & 77.21 $\pm$ 0.15 & 00.00 $\pm$ 0.00 & 0.00 
    & 48.70 $\pm$ 0.18 & 25.29 $\pm$ 1.53 & 0.00 \\
    TRADES + WAT & 80.38 $\pm$ 0.36 & 68.88 $\pm$ 2.40 & 0.07 
    & 46.95 $\pm$ 0.33 & 28.84 $\pm$ 1.34 & 0.41 \\    
    \midrule[.05em]
    TRADES + Ours & 81.58 $\pm$ 0.28 & 66.87 $\pm$ 1.02 & 0.02 
    & \textbf{49.16 $\pm$ 0.25} & \textbf{30.71 $\pm$ 1.19} & \textbf{0.46} \\
\midrule[.1em]
\end{tabular}
\label{tab:experiment_main}
\end{table}
